Designing with Deception: ML- and Covert Gate-Enhanced Camouflaging to Thwart IC Reverse Engineering

Integrated circuits (ICs) are essential to modern electronic systems, yet they face significant risks from physical reverse engineering (RE) attacks that compromise intellectual property (IP) and overall system security. While IC camouflage techniques have emerged to mitigate these risks, existing approaches largely focus on localized gate modifications, neglecting comprehensive deception strategies. To address this gap, we present a machine learning (ML)-driven methodology that integrates cryptic and mimetic cyber deception principles to enhance IC security against RE. Our approach leverages a novel And-Inverter Graph Variational Autoencoder (AIG-VAE) to encode circuit representations, enabling dual-layered camouflage through functional preservation and appearance mimicry. By introducing new variants of covert gates -- Fake Inverters, Fake Buffers, and Universal Transmitters -- our methodology achieves robust protection by obscuring circuit functionality while presenting misleading appearances. Experimental results demonstrate the effectiveness of our strategy in maintaining circuit functionality while achieving high camouflage and similarity scores with minimal structural overhead. Additionally, we validate the robustness of our method against advanced artificial intelligence (AI)-enhanced RE attacks, highlighting its practical applicability in securing IC designs. By bridging the gap in mimetic deception for hardware security, our work sets a new standard for IC camouflage, advancing the application of cyber deception principles to protect critical systems from adversarial threats.

==> settings.tches.tex <==
\setfirstpage{0}
\setlastpage{0}
\setvolume{0}
\setnumber{0}

\setISSN{2569-2925}
\makeatletter
\setDOI{10.46586/tches.v\IACR@vol.i\IACR@no.\IACR@fp-\IACR@lp}
\makeatother

\setkeys{IACR}{journal=tches}


==> settings.tosc.tex <==
\setfirstpage{0}
\setlastpage{0}
\setvolume{0}
\setnumber{0}

\setISSN{2519-173X}
\makeatletter
\setDOI{10.46586/tosc.v\IACR@vol.i\IACR@no.\IACR@fp-\IACR@lp}
\makeatother

